Interpretable Almost Matching Exactly for Causal Inference

We aim to create the highest possible quality of treatment-control matches for categorical data in the potential outcomes framework. Matching methods are heavily used in the social sciences due to their interpretability, but most matching methods do not pass basic sanity checks: they fail when irrelevant variables are introduced, and tend to be either computationally slow or produce low-quality matches. The method proposed in this work aims to match units on a weighted Hamming distance, taking into account the relative importance of the covariates; the algorithm aims to match units on as many relevant variables as possible. To do this, the algorithm creates a hierarchy of covariate combinations on which to match (similar to downward closure), in the process solving an optimization problem for each unit in order to construct the optimal matches. The algorithm uses a single dynamic program to solve all of the optimization problems simultaneously. Notable advantages of our method over existing matching procedures are its high-quality matches, versatility in handling different data distributions that may have irrelevant variables, and ability to handle missing data by matching on as many available covariates as possible.

==> sections/ActiveSetGenerationSection.tex <==
%A main goal of collapsing FLAME is to match on as many covariates as possible in order to reduce the distance between matched units. This goal is achieved by developping a scheme that solves the AEMR problem. We discuss this below.\\
Let us discuss the active set generation. Once we have identified the covariate-set to process during the first step of Collapsing FLAME, and saved the found main matched groups when we drop that set of covariates, we dynamically find the possible sets that can be processed at the next round of the algorithm. The essential algorithmic question is how to find all the covariate-sets that can be processed in a computationally tractable manner. A straightforward solution would be to test all $2^{|\mathcal{J}|}$ possible combinations of covariates at each round. This is unsustainable, as the number of possible combinations grows exponentially in the number of covariates. Also, the monotonicity property enforces that a large number of those combinations are not valid. For example, if  $\{1\}$ is the only processed set, it is unnecessary to test whether $\{1,2,3\}$ can be processed next because the monotonicity property requires  $\{1,2\}$, $\{1,3\}$ and $\{2,3\}$ to have been already processed. So, we use the monotonicity property to establish a hierarchical order in which to process covariate-sets. An \textit{active} set $s$ of  size $|s|$ covariates is defined to be a covariate-set for which all of its subsets of size $|s|-1$ were previously processed.  At each round, new combinations become active. 
%We note that solving AEMR is equivalent to finding all active covariate-sets subset of $\mathcal{J}$ that produce matched groups. Indeed, 
%\begin{proposition}{} Let $s$ be a covariate-set. Then,\\
%\[ \{ s \text{ is active and units were matched by dropping } s \} \iff  \vv \text{ is feasible} \]
%\textcolor{red}{I moved this from the beginning of the section to here}
%\end{proposition}

%\textcolor{red}{Working backwards,} suppose we are considering dropping covariate-set, the monotonicity property enforces that $\{1,2\}, \{1,3\}, \{2,3\}$ need to have been dropped in previous rounds. Iteratively, for $\{1,2\}$ to have been dropped, $\{1\}$ and $\{2\}$ need to have been dropped and so on. %\textcolor{red}{I do not understand what is happening from HERE}We denote {\it candidate} covariate-set, the combinations of covariate that are considered \textcolor{red}{where/when are these being considered? Are these the covariates that can now be dropped?}. Candidate sets need to verify certain properties that we will establish. For any candidate covariate-set, the iterative process in which it was created  means it is sufficient only to look at the one size less combinations of its covariate.\textcolor{red}{to HERE} Thus, the immediate {\it $k$-{subset}} definition: 
%{\bf Notations: } 
In this section, we denote $\Delta^k$ as the set of all $k$-sized processed covariate-sets, and $\Lambda_{(i)}$ denotes the set of all active sets at round $i$ of the Collapsing FLAME algorithm. $\Lambda_{(i)}$ needs to be updated at each round $i$ to include new active sets. Any combination of covariates we evaluate to be active is called a {\bf \it candidate}. Candidate sets need to satisfy certain conditions to be active sets. \\
Each time a covariate-set $\delta$ is processed, it is added to $\Delta^{|\delta|}$. To find the sets that become active, candidates can be formed as combinations of $|\gamma|+1$ covariates present in the union of covariate-sets in $\Delta^{|\delta|}$. 
%\begin{proposition}[Naive Candidates]
%Let $\delta_i$ be a newly processed set at round $i$ of collapsing FLAME. Let $\Gamma$ = $\{ \gamma \mid  \gamma \in \delta$ and $\delta \in \Delta^{|\delta_i|} \}$ be all the covariates that belong to a set of $\Delta^{|\delta_i|}$. Then, \\
%\[ \text{generate all } |\delta_i|+1 \text{ combinations of elements of } \Gamma:\]
%\[  \mathcal{C}^{naive} = \{ \{ \gamma_{\pi_{(1)}},...,\gamma_{\pi_{(|\delta_i|+1)}} \}, \text{where } \pi \text{is a permutation function} \} \]
%\end{proposition}
However, such method would generate too many superfluous candidates. Indeed, for any covariate that is not frequent enough in $\Delta^{|\delta|}$, the monotonicity property ensure that any candidate that contain that covariate is not valid. Suppose the previously processed sets of size 2 are $\{1,2\}, \{1,4\},\{1,5\}$ and the newly dropped set is $\{2,3\}$. Then, trying the combinations $\{1,2,4\}$ or $\{2,4,5\}$ is apriori unnecessary because $4$ and $5$ are not frequent enough. To formally define the frequency of a covariate, we introduce the notion of $support$.   
\begin{definition}[Support in $\Delta$: $\mathcal{S}_{\Delta}^e$] 
The support in $\Delta$ of a covariate $\mathbf{e}$ is the number of sets of $\Delta$ that contain $\mathbf{e}$: $\mathcal{S}_{\Delta}^e = \# \{ \delta \subset \Delta^{|\delta|}  \mid e \in \delta \}$
\end{definition}
\vspace{-2mm}
Using $support$, we propose to dynamically generate the set of candidates as follows: 
\vspace{-2mm}
\begin{proposition}[Candidates Generation] Let $\delta_i$ a newly dropped set at round $i$ of collapsing FLAME.
Let $\Gamma$ = $\{\gamma \mid  \gamma \in \delta$ and $\delta \in \Delta^{|\delta_i|} \setminus \delta_i \}$. Then, \\
if each covariate in $\delta_i$ have a support of at least $|\delta_i|$, generate candidates
\[ \mathcal{C} = \{ \delta_i \cup \gamma \mid \mathcal{S}_{\Delta^{|\delta_i|}}^\gamma \geq |\delta_i|, \textrm{\rm where  } \gamma \in \Gamma\}.\]
\end{proposition}
That is, take the union of the newly processed set $\delta_i$ with all the covariates that belong to a set in $\Delta^{|\delta_i|}$ and that have support of at least $|\delta_i|$. 

\begin{theorem}  (1) $\mathcal{C}$ contains all new active sets and (2) active sets are found as soon as they become active
\end{theorem}

Now that candidates have been generated, we need to find the candidates that are active. That consist in verifying, for each candidate $c$, if all its subsets of size $|c|-1$ have been processed.
%\begin{proposition}[Condition for activeness] Let $\delta_i$ be the dropped set at round $i$. \\
%Let $\mathcal{C}$ be the set of candidates that was generated. Then,
%\[ c \in \mathcal{C}  \text{ is active if and only if all  } |\delta_i|\text{-subsets of } c \text{ have been processed.} \],
%where a $k$-{subset} is a subset of size $k$ of $c$
%\end{proposition}
%\vspace{-2mm}
Finally, the set of active sets $\Lambda_{(i)}$ is updated with the newly active sets: 
\[ \Lambda_{(i+1)} = \Lambda_{(i)} \cup \{c \in \mathcal{C}  \mid  c   \text{ is active} \}\] 
\vspace{-6mm}
\begin{theorem}\textrm{(Correctness)}
Collapsing FLAME where all units are reused solves the AEMR problem for every treatment and control unit $i$. 
\end{theorem}
(See appendix for proofs of theorems)

Algorithm \ref{alg:generatenewactivesets} shows the procedure for generating new active sets as well as an example. A more complex example is detailed in the appendix
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
  \caption{Procedure {\it \GenerateNewActiveSets \label{alg:generatenewactivesets}}  $ \mid $  {\bf Example} }
  \begin{multicols}{2}
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}  

    \Input{ $\nu$ a newly dropped set of size $k$,\\ $\Delta $ the set of previously processed sets }
    
    {\bf Initialize: }  \texttt{\rm \small new active sets} $Z$ = $\emptyset$ 

    \texttt{\rm \small -- add $\nu$ in $\Delta^k $} 
    
    $\Delta^k$ = $\{\delta \in \Delta \; \mid \; size(\delta) = k \} \cup \{\nu\}$
    
    {\bf Notation: } $\mathcal{S}_{\Delta^k}^e$ = support of covariate $e$ in $\Delta^k$ 
    
    \texttt{\rm \small -- get all the covariates contained in sets in $\Delta^k $} 
    
    $\Gamma$ = $\{\gamma \; \mid \; \gamma \in \delta$ and $\delta \in \Delta^k \}$ 
    
    \texttt{\rm \small -- get the covariates that have enough support minus $\nu$} 
    
    $\Omega$ = $\{\alpha \; \mid \; \alpha \in \Gamma$ and $\mathcal{S}_{\Delta}^e \geq k \} \setminus \nu\ $ 
         
      \textrm{\rm  \small -- if all covariates in $\nu$ have enough support in $\Delta^k$} 
      
      \If{$\{\forall e \in \nu : \mathcal{S}_{\Delta^k}^e \geq k \}$   }{
      
          \texttt{\rm \small -- generate candidate set $\nu \cup \{\alpha\}$ for $\alpha \in \Omega  $ }
                    
          \For{ all $\alpha \in \Omega$ }{
          
              $c = \nu \cup \{\alpha\} $
          
              \If{all $k$-subset of $c \in \Delta^k$ }{
           
              \texttt{\rm \small -- add newly active set $c$ to $Z$}
          
              add $c$ to $Z$ 
              } 
           }   

      }
%         \EndIf
 


     \KwRet{$Z$}
     

     $\nu = \{2,3\}$, $k=2$, \\ $\Delta = \{ \{1\}, \{2\}, \{3\}, \{1,2\},
     \{1,3\} \}$ 
    
     $Z$ = $\emptyset$  
     \linebreak
    
    $\Delta^2$ = $\{\{1,2\},\{1,3\},\{2,3\} \}$ 
    
    $\mathcal{S}_{\Delta^2}^1 = 2, \mathcal{S}_{\Delta^2}^2 = 2, \mathcal{S}_{\Delta^2}^3 = 2$
    \linebreak

    $\Gamma$ = $\{1,2,3 \}$ 
    \linebreak
    
    $\Omega$ = $\{1,2,3 \} \setminus \{2,3\} = \{1\}$
    \linebreak 
       
      $True:$
      \linebreak
          
          $\alpha = 1 $
                   
          $c = \{2,3\} \cup \{1\} = \{1,2,3\}$
          
          $True$ ($2$-subset of $c$ are $\{1,2\},\{1,3\},\{2,3\})$
          \linebreak
          
              $ Z = \{\{1,2,3\}\}$ 
              \linebreak
      
%         \EndIf
 



     \KwRet{ $Z = \{\{1,2,3\}\}$}
     
     
     \end{multicols}

\end{algorithm}
\end{minipage}

%{\bf Example:}
%\begin{wrapfigure}{r}{0.7\textwidth}
%  \begin{center}
%    \includegraphics[width=0.7\textwidth]{example}
%  \end{center}
%  \caption{Example of the first few steps of Collapsing FLAME for a dataset with 3 covariates}
%\end{wrapfigure}

% \input{active_sets_example}

%Figure 2 shows an example of collaping FLAME for a dataset with three covariates. The descending arcs ({\it newly dropped set}) implicitly represent {\bf Step 1 } of the algorithm that finds which best active set to drop. Then, the {\it newly dropped set} is added in the right $\Delta^k$. The ascending arcs ({\it new active set}) represent {\bf Step 2} where new active set are found. If new sets become active, add them to the set of active sets. Otherwise, do nothing. This procedure is repeated until no matches are possible or there are no remaining active sets.

%This algorithm returns the near optimal matched groups on the Hamming distance from the input dataset of treatment and control units.
%\end{wrapfigure}


%$\bullet$ Collapsing + generic FLAME = linear model

To facilitate matching with replacement as in the AEMR objective and to keep track of main and auxiliary matched groups, the algorithm uses a variant of \BasicExactMatch\ given in Algorithm~\ref{algo:basicexactmatch} (denoted by \BasicExactMatch*\). In an iteration $i$, the  \BasicExactMatch$^*$ procedure takes the entire set of units $D$, the set of unmatched units from the previous iteration $D_{(i-1)}$, and the covariate-set $J \setminus s_{(i)}^*$ to match on in this iteration (the discussion on how the best active set )


==> sections/BasicExactMatch.tex <==
\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{Unmatched Data $D^{um} =(X,Y,T)$, subset of indexes of covariates $J^s \subseteq\{1,...,p\}$.}
    \Output{Newly matched units $D^m$ using covariates indexed by $J^s$ where groups have at least one matched and one control unit, the remaining data as $D^{um} \setminus D^m$ and matched groups for $D^m$.}
    %Let $X_{J^s}$ = the subset of covariates indexed by $J^s$\\
    $M_{raw}$=\texttt{group{-}by} $(D^{um}, J^s)$ (\tt \small form groups by exact matching on $J^s$)\label{step:basic-1}\\ %(D,X(:,J))$\\
    $M$=\texttt{prune}($M_{raw}$) ({\tt \small remove groups without at least one treatment and control unit})\label{step:basic-2}\\
%    Attach a group-id to each group of $M$\\
    $D^m$=Get subset of $D^{um}$ where the covariates match with $M$ \texttt{\small (recover newly matched units)}\label{step:basic-3}\\
     \Return{$\{D^m, D^{um} \setminus D^m, M\}$. ({\tt matched units, unmatched units, and matched groups})}
    \caption{Procedure {\BasicExactMatch}}
    \label{algo:basicexactmatch}
\end{algorithm}
    \vspace{-10pt}




==> sections/feasible_sets_example.tex <==
\vspace{-2mm}
\begin{algorithm}
  \caption{Procedure {\it GenerateNewFeasibleSets}}
  % \begin{multicols}{2}
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}  

    \Input{ $\nu$ a newly dropped set of size $k$,\\ $\Delta $ the set of previously dropped sets }
    
    {\bf Initialize: }  \texttt{\rm \small new feasible sets} $Z$ = $\emptyset$ 
    
    $\Delta^k$ = $\{\delta \in \Delta \; \mid \; size(\delta) = k \}$
    
    {\bf Notation: }$\forall$ feature $e$, $\mathcal{S}_{\Delta^k}^e$ = support of $e$ in $\Delta^k$ 
    
    \texttt{\rm \small -- get all the features contained in sets in $\Delta^k $} 
    
    $\Gamma$ = $\{\gamma \; \mid \; \gamma \in \delta$ and $\delta \in \Delta^k \}$ 
    
    \texttt{\rm \small -- get all the features that have minimum support} 
    
    $\Omega$ = $\{\alpha \; \mid \; \alpha \in \Gamma$ and $\mathcal{S}_{\Delta}^e \geq k \}$ 
    
    \texttt{\rm \small -- add $\nu$ to $\Delta^k$ which updates the support of $e \in \nu $} 
    
    $\Delta^k$ = $\Delta^k \cup \{\nu\}$  
 
      \textrm{\rm  \small -- if all features in $\nu$ have minimum support in $\Delta^k$} 
      
      \If{$\{\forall e \in \nu : \mathcal{S}_{\Delta^k}^e \geq k \}$   }{
      
          
          \texttt{\rm \small -- generate candidate set $\nu \cup \{\alpha\}$ for $\alpha \in \Omega  $ }
          
          $c = \nu \cup \{\alpha\} $
          
          \If{ $k$-subset of $c \in \Delta^k$ }{
           
              \texttt{\rm \small -- add newly feasible set $c$ to $Z$}
          
              add $c$ to $Z$ 
              } 

      }
%         \EndIf
 


     \KwRet{$Z$}     
     
     % \end{multicols}

\end{algorithm}

{\bf Example:} Given the initial active-sets, solve the optimization problem $(1)$ to find the feasible feature-set (denoted ${\it newly dropped set}$) that maximizes the match quality. 

\noindent\begin{minipage}{.3\textwidth}
  \begin{algorithm}
   \caption{Procedure {\it GenerateNewFeasibleSets}}
    % \SetKwInOut{Input}{Input}
    % \SetKwInOut{Output}{Output}  
    \Input{ $\nu$ a newly dropped set of size $k$,\\ $\Delta $ the set of previously dropped sets }

    $\nu = \{2,3\}$, $k=2$, \\ $\Delta = \{ \{1\}, \{2\}, \{3\}, \{1,2\}, \{1,3\} \}$ 
    
    $Z$ = $\emptyset$  
    
    $\Delta^2$ = $\{\{1,2\},\{1,3\} \}$ 
    
    $\mathcal{S}_{\Delta^2}^1 = 2, \mathcal{S}_{\Delta^2}^2 = 1, \mathcal{S}_{\Delta^2}^3 = 1, \mathcal{S}_{\Delta^1}^1 = 1$
    \linebreak

    $\Gamma$ = $\{1,2,3 \}$ 
    \linebreak
    
    $\Omega$ = $\{1\}$
    \linebreak
    
    $\Delta^2$ = $\{\{1,2\},\{1,3\},\{2,3\}\}$  \texttt{\rm \small ($\mathcal{S}_{\Delta^2}^2 = 2, \mathcal{S}_{\Delta^2}^2 = 2$)}
    \linebreak 
       
      $True:$
      \linebreak
          
          $c = \{2,3\} \cup \{1\} = \{1,2,3\}$
          
          $True$ ($2$-subset of $c =  \{\{1,2\}, \{1,3\}, \{2,3\}\}$
          \linebreak
          
              $ Z = \{\{1,2,3\}\}$ 

      
%         \EndIf
 



     \KwRet{ $Z = \{\{1,2,3\}\}$}

  \end{algorithm}


\end{minipage}
\begin{minipage}{.7\textwidth}
\includegraphics[width=0.7\textwidth]{example.pdf}  
{Example of the first few steps of Collapsing FLAME for a dataset with 3 features}
% \begin{figure}{0.7\textwidth}
%   \begin{center}
%     \includegraphics[width=0.7\textwidth]{example.pdf}
%   \end{center}
%   \caption{Example of the first few steps of Collapsing FLAME for a dataset with 3 features}
% \end{figure}
\end{minipage}


==> sections/group-by.tex <==
% \section{The Procedure and its implementation using bit-vectors}
\section{Bit-vector implementation details}
\label{sec:group-by}
%{Yameng will work on this.}

\cut{
\section{Database queries: \texttt{group-by}}
\texttt{group-by} is a powerful database query available on most relational database management systems. Distinctive features of database queries are (1) their scalabilty to large dataset that can not fit in memory, (2) a high level syntax that allow for an intuitive call to complex operations. For example, finding covariates units matched on can be achieved in one line (see below). Utilizing robust database queries to scale causal inference methods is an emerging field of study (see \citep{SalimiCPS17}). In \BasicExactMatch\  the exact matching step can succintly be computed using  \texttt{group-by}:\\
{\small \tt

WITH tempgroups AS \\
       (SELECT \(A\sb{1}, A\sb{2}, \cdots, A\sb{p}\) \hspace*{10pt}\textrm{ (matched groups are identified by their covariate values)}\\
       FROM D\\
       WHERE  \(\ismatched\ = 0\) \hspace*{10pt}\textrm{ (use data that are not yet matched)}\\
       GROUP BY \(A\sb{1}, A\sb{2}, \cdots, A\sb{p}\) \hspace*{10pt}\textrm{ (create matched groups with identical covariates)} \\
       HAVING SUM(T) >= 1 AND SUM(T) <= COUNT(*)-1 \hspace*{10pt}\textrm{(groups have}\(\geq\)\textrm{1 treated, but not all treated)} \\
       \\
}      
{\bf Notations:} A new column is added to the input dataset to identify units that have been matched. Each time a unit is matched, the value of $\ismatched\ $ for that unit is set to $1$. Conversely, the unmatched units have a $\ismatched\ $ set to $0$. $A_1, \cdots, A_p$ are the covariates in $\mathcal{J}$. The \emph{SELECT, WHERE, GROUP-BY clauses} go through the covariates of the input dataset $D$ (SELECT), indentify units that have not been matched yet (WHERE) and finds the covariates on which those units matched on. The \texttt{pruning} step (HAVING clause) ensures that the constraint of at least one treatment and one control unit in the matched groups be satisfied. \text{\it tempgroups} temporarily contains all groups found. \\

Once the matched groups are found, the dataset of all units is updated with (1) the newly matched units that are replaced inplace by their values in tempgroups and (2) the updated $\ismatched\ $ indicator for those units.\\
{\small \tt
SET \(\ismatched\ = \ell\) \\
WHERE  EXISTS \\
   \ SELECT \(D.A\sb{1}, D.A\sb{2}, \cdots, D.A\sb{p}\) \\
    FROM tempgroups S \hspace*{10pt}\textrm{(set of covariate values for valid groups)} \\
    WHERE  \(S.A\sb{1} = D.A\sb{1}\) AND \(S.A\sb{2} = D.A\sb{2}\) AND \(\cdots\) AND \(S.A\sb{p} = D.A\sb{p}\) \\
    \\
    AND \(\ismatched\ = 0\) \\
}


}
\textcolor{red}{alex: we can drop this section completely. It introduces a bunch of notation that is never used again. In section 4 after we introduce alg2 we can add ``A detailed exposition of the bit-vector implementation is available in Wang et al''}
We implement the ``Group-by'' operation by bit-vector manipulation \citep{genericFLAME2017}. Assume there are $p$ covariates in the dataset. If the $i$-th  covariate is $k_{(i)}$-ary ($k_{(i)} \ge 2$), we at first rearrange the $p$ covariates such that $k_{(i)} \ge k_{(i+1)}$ for all $0 \le i \le p-2$ and get reordered covariates values of unit $u_i$ to be $(a_{p-1}, a_{p-2}, \dots, a_0)$. Then for each unit $u$, we compute two values: 
$ b_u = \sum_{j=0}^{q-1} a_j k_{(j)}^j $
together with the treatment indicator value $T = t$,
 $ b_u^+ = t + \sum_{j=0}^{p-1} a_j k_{(j)}^{j+1}$ \\
 
Since the covariates are rearranged so that $k_{(i)} \le k_{(i+1)}$ for all $0 \le i \le p-2$, two units $u$ and $u'$ have the same covariate values if and only if $b_u = b_{u'}$. For each unit u with values $b_u$ and $b_u^+$, we compute how many times these two values occurs for all the units in the dataset (using unique() function of Numpy package in Python) and denote them as $c_u$ and $c_u^+$ respectively. To guarantee each matched group has at least one treatment and one control, we mark a unit $u$ as matched if its $c_u$ and $c_u^i$ differs. A rigorous proof can be found in \cite{genericFLAME2017}.


==> sections/ref.tex <==
%\section*{References}
%\bibliographystyle{plain}
\bibliographystyle{abbrvnat}
%\bibliography{refrences/biblio}
\bibliography{biblio}
%\input{main.bbl}

==> sections/timing.tex <==
\section{Simulations}
\label{sec:Timing}

\begin{wrapfigure}{R}{7cm}
    \vspace{-.5cm}
    \centering
    \includegraphics[width=.5\textwidth]{415timing.png}
     %\caption{The ExoPlex network service architecture. ExoPlex is a vSDX with an elastic slice controller that exposes an API to clients, and uses a SAFE engine to check incoming requests for compliance with a logical trust policy.}
     \caption{Running time comparison}
     \vspace{-.1cm}
 \end{wrapfigure}
 
We study the running time of the different methods for different dataset sizes. Generic FLAME provides the best running time performance because it utilizes the bit vector implementation and incrementally decrease the covariate space. Collapsing FLAME resets the pool of covaraite-sets to consider at each round of the algorithm. It achieves lower performance compared to the other methods. However, as shown in the previous simulations, collapsing FLAME produces high quality matches that the other methods do not. The running time can be optimized through parallelization. Indeed, testing of all possible sets to find the best on to process is easily parallizable and would improve the running time.
